ForgeMegakernel: A General Framework for Efficient Auto-Regressive Model Decode Megakernels

Auto-regressive model decode is bandwidth-bound, since every weight and key/value-cache byte crosses high-bandwidth memory once per token. A megakernel is an ideal solution, but existing automatic megakernel generation approaches cannot achieve both generalization across models and correctness guarantees. We present ForgeMegakernel, which generates a per-model high-performance decode megakernel using coding agents. ForgeMegakernel pairs a universal knowledge base of ten progressive milestones with an independent mid-state test oracle. The milestones provide the megakernel's structural properties: a fine-grained instruction stream for each SM, dependency counters replacing the global synchronization, and a shared-memory buffer pool for workload balance across SMs and greater parallelism. The test oracle derives the mid-states of the megakernel and checks the performance, error and precision during the generation process, guaranteeing a correct and trustworthy forged megakernel. We evaluated ForgeMegakernel on 14 representative decoding operations across eight model families spanning 0.6B-13B parameters. The generated megakernels achieved 50.5-85.9% MBU and geometric mean speedups of 1.21x over SGLang 0.5.18 and 1.54x over a megakernel compiler under identical configurations. Inside SGLang, evaluated on GSM8K with ragged prompts, all 14 megakernels decoded faster than the SGLang engine at comparable answer accuracy.

==> sec/fig-acc.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/fig_acc.pdf}
\caption{Error against exact arithmetic: both decoders
teacher-forced on the same prompts, their next-token top-1 choices compared to a
float64 forward's. Lower is closer to the truth.}
\label{fig:acc}
\end{figure}


==> sec/fig-obs31.tex <==
\begin{figure}[t]
\centering
\includegraphics{figs/fig_obs31.pdf}
\caption{One session against a relay, on one configuration (Qwen3-0.6B,
$b1{\times}128$), from one scaffold commit. \textbf{(a)} the highest milestone an
artefact holds against the agent sessions spent on it: a single-pass attempt is
one session, a relay replicate one session per round. Same tools, same rules,
same agent --- the relay is the variable. \textbf{(b)} MBU relative to the configuration's measured ceiling. The re-tune experiments are handed a forged megakernel and asked for
context~2048, so they begin where the build ends.}
\label{fig:obs31}
\end{figure}


==> sec/tab-cells.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2.0pt}
\caption{The 14 forged megakernels: the decode step in isolation
(left) and the same kernel as an SGLang model class (right). A row shares
the numerator of \eqcite{eq:bytes}, so an MBU ratio is a latency ratio. \emph{hand} is
our reproduction of a hand-written megakernel~\cite{spector2025nobubbles};
\emph{golden} is top-1 agreement with a float64 forward and \emph{acc} no worse
than the SGLang engine on decidable positions, both dashed where no teacher-forced pass
exists. $\ddagger$~speed reference, untrained checkpoint, in no mean.}
\label{tab:cells}
\begin{tabular}{@{}lrrrrrrrrrrrrrrrrl@{}}
\toprule
& & & \multicolumn{9}{c}{\textbf{decode step in isolation}} & \multicolumn{6}{c}{\textbf{inside the SGLang serving engine}} \\
\cmidrule(lr){4-12}\cmidrule(lr){13-18}
& & & \multicolumn{2}{c}{Ours} & SGL & MPK & vLLM & llm.cpp & hand & \multicolumn{2}{c}{vs} & \multicolumn{2}{c}{Ours} & baseline & & top-1 vs \\
\cmidrule(lr){4-5}\cmidrule(lr){11-12}\cmidrule(lr){14-15}
Model & $b$ & $S$ & \us & MBU & MBU & MBU & MBU & MBU & MBU & SGL & MPK & \us & MBU & MBU & speed & golden & acc \\
\midrule
Qwen3-0.6B & 8 & 2048 & 1648 & \textbf{55.6\%} & 40.6\% & 30.6\% & 38.8\% & 16.2\% & -- & 1.37$\times$ & 1.82$\times$ & 2012 & \textbf{45.6\%} & 40.6\% & 1.12$\times$ & 0.9987 & \checkmark \\
Qwen3-0.6B & 16 & 1024 & 1814 & \textbf{50.5\%} & 40.2\% & 20.6\% & 38.2\% & 10.1\% & -- & 1.26$\times$ & 2.45$\times$ & 2246 & \textbf{40.8\%} & 40.9\% & 1.00$\times$ & 0.9973 & \checkmark \\
Qwen3-0.6B & 16 & 4096 & 3396 & \textbf{76.6\%} & 64.1\% & 29.3\% & 61.8\% & 24.1\% & -- & 1.19$\times$ & 2.61$\times$ & 3733 & \textbf{69.6\%} & 64.2\% & 1.08$\times$ & 0.9993 & \checkmark \\
Qwen3-4B & 1 & 128 & 3233 & \textbf{74.5\%} & 61.0\% & 54.0\% & 55.9\% & 50.7\% & -- & 1.22$\times$ & 1.38$\times$ & 3710 & \textbf{64.9\%} & 64.0\% & 1.01$\times$ & 0.9980 & \checkmark \\
Qwen3-4B & 8 & 1024 & 4254 & \textbf{64.9\%} & 57.3\% & 52.3\% & 57.5\% & 32.1\% & -- & 1.13$\times$ & 1.24$\times$ & 4708 & \textbf{58.7\%} & 57.0\% & 1.03$\times$ & 0.9978 & \checkmark \\
Qwen3-8B & 1 & 128 & 5432 & \textbf{83.3\%} & 72.8\% & 70.2\% & 67.9\% & 67.8\% & -- & 1.14$\times$ & 1.19$\times$ & 5771 & \textbf{78.4\%} & 74.4\% & 1.05$\times$ & 0.9941 & \checkmark \\
Qwen3-8B & 1 & 512 & 5485 & \textbf{82.8\%} & 72.0\% & 64.5\% & 69.8\% & 67.7\% & -- & 1.15$\times$ & 1.28$\times$ & 5858 & \textbf{77.5\%} & 74.0\% & 1.05$\times$ & 0.9912 & \checkmark \\
Qwen3-8B & 1 & 2048 & 5730 & \textbf{80.4\%} & 72.1\% & 53.5\% & 69.9\% & 66.7\% & -- & 1.12$\times$ & 1.50$\times$ & 6152 & \textbf{74.9\%} & 73.4\% & 1.02$\times$ & 0.9923 & \checkmark \\
\addlinespace
Llama-3.1-8B & 4 & 2048 & 6105 & \textbf{78.7\%} & 69.7\% & 61.6\% & 69.5\% & 54.6\% & -- & 1.13$\times$ & 1.28$\times$ & 6535 & \textbf{73.5\%} & 70.8\% & 1.04$\times$ & 0.9999 & \checkmark \\
Llama-2-13B-chat & 1 & 128 & 8971 & \textbf{85.9\%} & 78.9\% & 75.9\% & 74.2\% & 72.8\% & -- & 1.09$\times$ & 1.13$\times$ & 9479 & \textbf{81.3\%} & 79.1\% & 1.03$\times$ & 0.9961 & \checkmark \\
\addlinespace
MiniCPM5-1B & 1 & 128 & 898 & \textbf{58.6\%} & 36.5\% & 30.9\% & 31.2\% & 24.8\% & -- & 1.61$\times$ & 1.89$\times$ & 1216 & \textbf{43.3\%} & 37.1\% & 1.17$\times$ & 0.9961 & \checkmark \\
MiniCPM4-1B & 1 & 128 & 1563 & \textbf{56.3\%} & 45.2\% & 39.7\% & 39.8\% & 38.5\% & -- & 1.24$\times$ & 1.42$\times$ & 1711 & \textbf{51.4\%} & 45.4\% & 1.13$\times$ & 0.9921 & \checkmark \\
MiniCPM4-3B & 1 & 128 & 2830 & \textbf{72.1\%} & 61.7\% & 46.9\% & 53.6\% & 52.5\% & -- & 1.17$\times$ & 1.54$\times$ & 3162 & \textbf{64.6\%} & 64.3\% & 1.00$\times$ & 0.9980 & \checkmark \\
\midrule
Llama-3.2-1B$^{\ddagger}$ & 1 & 96 & 998 & \textbf{74.0\%} & 53.9\% & 48.7\% & 49.2\% & 40.3\% & \textbf{74.6\%} & 1.37$\times$ & 1.52$\times$ & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{10}{r}{geometric mean\quad} & \textbf{1.21$\times$} & \textbf{1.54$\times$} & & & & \textbf{1.06$\times$} & & \\
\bottomrule
\end{tabular}
\end{table*}


==> sec/tab-defects.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\caption{Ways a round measured well and was wrong anyway, over
the 1{,}277 rounds mined for defects. Row E is the class \sys{} still does not
cover.}
\label{tab:defects}
\begin{tabular}{@{}p{0.145\textwidth}p{0.415\textwidth}p{0.375\textwidth}@{}}
\toprule
\textbf{Class} & \textbf{Observed instance} & \textbf{Countermeasure in \sys} \\
\midrule

\textbf{A. The measured path is not the shipped path}
& The binding layer picks its execution path from the calling gate's stack frame
and the end-to-end milestone is not in the fused set, so every historic
``\code{abs\_err 0.00e+00}'' from it describes a PyTorch scaffold on real
weights. Separately, a kernel with four narrowed arithmetic sites reported a
green width ratio because the operator entry points the gate called were
standalone kernels sharing no arithmetic with the fused path.
& Milestones \rung{M5}--\rung{M9} re-run all numerics on the kernel that milestone just
built; \code{op\_*} must route through the fused path from \rung{M5} on; the
launch count is a structural milestone, not a self-report. \\
\addlinespace

\textbf{B. The metric rewards the wrong artefact}
& Accuracy scored against a bf16 reference pays for extra roundings: one agent
moved its rotary table to bf16 and spelled the norm gain and SwiGLU boundary in
native bf16, and its error metric \emph{fell}. An MBU numerator charging the whole
embedding table inflates utilization $1.22\times$ on untied models; we found this
over-count in two published systems' own reporting.
& Numerator derived from the config in one hashed module
(\S\ref{sec:design:oracle}); error scored against exact fp64 arithmetic;
arithmetic width judged by a separate regression onto the narrowing direction,
\eqcite{eq:alpha}. \\
\addlinespace

\textbf{C. The code read is not the code that ran}
& A \code{constexpr} inside an \code{\#if} evaluates to 0 rather than its
declared value --- three occurrences in one cell, whose honest re-measure was
$0.89\times$ rather than the reported speedup. An edit lands in the dead branch of an
\code{\#ifdef} chain and two rounds measure a build neither commit describes. A
ported predicate over the hidden size goes statically false and darkens a fast
path worth 479.5\us{} behind a legal launch.
& Every milestone prints the resolved value of each compile-time constant the build
used; the review round diffs the commit against that resolved header; a static
audit sweeps every worktree for shapes already seen. \\
\addlinespace

\textbf{D. The instrument lied}
& \emph{The environment}: three of eight cards on one host were clock-locked at
1590 rather than 1980\,MHz, so a cell's microseconds read low by that ratio,
and contention from an orphaned process measured byte-identical work at 4470\us{}
and 2015\us. \emph{The check itself}: the random-weight oracle set every norm gain
to \code{ones}, making the width judge's two reference variants bit-identical, so
it abstained by construction on half the configurations; and a relative error divided by a
near-zero reference read one bf16 unit in the last place as a $383\times$ error.
& Device clock and identity are gate-recorded per run and compared, and a claimed
win under the measured noise floor requires a same-session re-measure of the
identical build. An abstain is never converted to a pass and is reported as its own verdict; oracles
carry non-degenerate weights; in-kernel checks are validated on CPU with fault
injection before they gate anything. \\
\addlinespace
\midrule
\textbf{E. Not covered}
& The forced numerics checks only ever drive \emph{uniform} decode positions, so a
kernel that broadcasts one lane's position across a ragged batch
(\code{positions[0]} instead of per-lane) passes every milestone yet decodes other
lanes at the wrong position under a real serving batch --- the MiniCPM4-3B batched
configurations (b8 forged, b16 withheld) collapse to 0.025 GSM8K accuracy, and further
withheld batched configurations fail the same way.
& None. Separated only by a ragged in-engine batch (\S\ref{sec:eval:gsm8k}); the
defect is located and fixable but the isolation ladder cannot generate the input
that reveals it. \\
\bottomrule
\end{tabular}
\end{table*}


==> sec/tab-err.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.6pt}
\caption{Error against exact arithmetic, both decoders teacher-forced on the
same prompts against a float64 forward. \emph{decidable} drops the positions
whose top two golden logits sit within one bf16 ulp; $d_{\mathrm{TV}}$ is the
top-64 distance. Lower is closer.}
\label{tab:err}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
& & & \multicolumn{2}{c}{raw misses} & \multicolumn{2}{c}{decidable misses} & \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Model & cell & pos. & ours & SGLang & ours & SGLang & $d_{\mathrm{TV}}$ \\
\midrule
Qwen3-0.6B & $8{\times}2048$ & 8188 & \textbf{11} & 19 & \textbf{0} & 0 & 0.0177 \\
Qwen3-0.6B & $16{\times}1024$ & 4092 & \textbf{11} & 17 & \textbf{0} & 0 & 0.0113 \\
Qwen3-0.6B & $16{\times}4096$ & 16380 & \textbf{12} & 19 & \textbf{0} & 0 & 0.0163 \\
Qwen3-4B & $1{\times}128$ & 508 & \textbf{1} & 11 & \textbf{0} & 1 & 0.0419 \\
Qwen3-4B & $8{\times}1024$ & 4092 & \textbf{9} & 23 & \textbf{1} & 2 & 0.0264 \\
Qwen3-8B & $1{\times}128$ & 508 & \textbf{3} & 13 & \textbf{0} & 0 & 0.0087 \\
Qwen3-8B & $1{\times}512$ & 2044 & \textbf{18} & 45 & \textbf{1} & 5 & 0.0060 \\
Qwen3-8B & $1{\times}2048$ & 8188 & \textbf{63} & 127 & \textbf{1} & 8 & 0.0127 \\
\addlinespace
Llama-3.1-8B & $4{\times}2048$ & 8188 & \textbf{1} & 11 & \textbf{0} & 1 & 0.0047 \\
Llama-2-13B & $1{\times}128$ & 508 & \textbf{2} & 0 & \textbf{0} & 0 & 0.0149 \\
\addlinespace
MiniCPM5-1B & $1{\times}128$ & 508 & \textbf{2} & 10 & \textbf{0} & 0 & 0.0112 \\
MiniCPM4-1B & $1{\times}128$ & 508 & \textbf{4} & 4 & \textbf{0} & 0 & 0.0106 \\
MiniCPM4-3B & $1{\times}128$ & 508 & \textbf{1} & 4 & \textbf{0} & 0 & 0.0202 \\
\bottomrule
\end{tabular}
\end{table}


==> sec/tab-insertion.tex <==
% merged into tab-cells.tex


==> sec/tab-knobs.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Engine-baseline knob ladder (Qwen3-4B). Each delta is against that
engine's own control run on the same release, so the configuration is isolated
from the version bump. Two identical control runs differ by 0.09\%.}
\label{tab:knobs}
\begin{tabular}{@{}llrr@{}}
\toprule
Engine & Knob & $b1{\times}128$ & $b8{\times}1024$ \\
\midrule
SGLang & \code{enable\_torch\_compile} & +5.7\% & +1.5\% \\
SGLang & \quad + graph-batch knobs & +4.9\% & +1.2\% \\
SGLang & \code{cuda\_graph\_max\_bs}, \code{max\_running\_requests} & -4.5\% & -2.4\% \\
SGLang & \code{skip\_tokenizer\_init} & -4.9\% & -4.4\% \\
\addlinespace
vLLM & \code{V1\_MULTIPROCESSING=0} & +4.7\% & +3.5\% \\
vLLM & \quad + \code{detokenize=False} & +4.7\% & +3.7\% \\
vLLM & \code{detokenize=False} & +0.6\% & +2.6\% \\
vLLM & \code{max\_num\_seqs}, \code{max\_model\_len} & -0.2\% & -0.1\% \\
\bottomrule
\end{tabular}
\end{table}


==> sec/tab-oracle.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{The oracle by the question each quantity settles. Every one is fixed
from the model configuration before any kernel exists, which is what makes the
right-hand column unreachable from inside the kernel.}
\label{tab:oracle}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{0.215\columnwidth}>{\raggedright\arraybackslash}p{0.275\columnwidth}>{\raggedright\arraybackslash}p{0.42\columnwidth}@{}}
\toprule
\textbf{quantity} & \textbf{derived from} & \textbf{what it closes} \\
\midrule
\multicolumn{3}{@{}l}{\emph{How fast is this kernel?}}\\[1pt]
$B(b,S)$,
\eqcite{eq:bytes} & dimensions, dtype, the configuration $(b,S)$ & the kernel
supplying the bytes it is scored on; an inflated numerator crashes on
MBU $>100\%$ \\
read amplification & \code{ncu} DRAM reads over $B(b,S)$ & reading every weight
twice and calling the result low utilization \\
clock scope & declared per backend & ranking a kernel-only number against an
end-to-end one \\
two-point slope & $n = 16$ against $n = 80$ & prefill and every
length-independent term inside a per-token latency \\
\addlinespace
\multicolumn{3}{@{}l}{\emph{How wrong are its answers?}}\\[1pt]
float64 golden & the bf16 checkpoint upcast exactly & scoring error against a
PyTorch scaffold, or against a reference the kernel can converge toward \\
$\text{err} \le 5D$ & $D$, the bf16 reference's own distance from exact
arithmetic & a tolerance chosen by hand, and one that does not port across
models \\
\textsf{finite}, canary,
$C < 2B$ & forced from \rung{M5} up; no calibrated constant & an out-of-bounds
KV read that still produces plausible logits \\
\addlinespace
\multicolumn{3}{@{}l}{\emph{Is it holding the arithmetic width it claims?}}\\[1pt]
$\alpha \le 0.5$,
\eqcite{eq:alpha} & two references per boundary operator, from one tap &
fp32 activations spelled in bf16 to buy speed, inside a tolerance an order of
magnitude looser \\
\bottomrule
\end{tabular}
\end{table}


==> sec/tab-profile.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Decode-step profile, per token, end-to-end scope.
\emph{idle}: share of the step with no kernel resident; MPK reads 0.00 launches
because its kernels launch per burst. Each arm is its own session.}
\label{tab:profile}
\begin{tabular}{@{}llrrrr@{}}
\toprule
Cell & System & launches & \us/tok & MBU & idle \\
\midrule
\multirow{4}{*}{\shortstack[l]{MiniCPM5-1B\\$b1{\times}128$}}
 & \sys      & 2.00   & \textbf{1025} & \textbf{51.4} & 0.21\% \\
 & SGLang    & 280    & 1483 & 35.5 & 0.68\% \\
 & vLLM      & 311    & 1575 & 33.4 & 1.17\% \\
 & MPK       & 0.00   & 1867 & 28.2 & 0.20\% \\
\addlinespace
\multirow{4}{*}{\shortstack[l]{Qwen3-8B\\$b1{\times}128$}}
 & \sys      & 2.00   & \textbf{5707} & \textbf{79.3} & 0.08\% \\
 & SGLang    & 448    & 6043 & 74.9 & 0.00\% \\
 & vLLM      & 491    & 6615 & 68.4 & 1.74\% \\
 & MPK       & 0.00   & 6640 & 68.1 & 0.15\% \\
\bottomrule
\end{tabular}
\end{table}

